Tests of Conformal Invariance in Randomness Induced Second-Order Phase Transitions

The conformal covariance of correlation functions is checked in the second-order transition induced by random bonds in the two-dimensional 8-state Potts model. The decay of correlations is obtained {\it via} transfer matrix calculations in a cylinder geometry, and large-scale Monte Carlo simulations give access to the correlations and the profiles inside a square with free or fixed boundary conditions, respectively. In both geometries, conformal transformations constrain the form of the spatial dependence, leading to accurate determinations of the order parameter scaling index in good agreement with previous independent determinations obtained through standard techniques. The energy density exponent is also computed.

==> entete.tex <==
\input epsf.tex
\textheight 245mm
\setcounter{page}{1}
\pagestyle{plain}
\makeatletter
\def\refrule{%
\end{multicols}\widetext\vglue13pt %
\hskip10.25pc\rule{20pc}{.1mm}\hfill %
\vglue.14cm\begin{multicols}{2}\narrowtext %
}

\def\references{%
\list{\@biblabel{\arabic{enumiv}}}%
{\labelwidth\WidestRefLabelThusFar  \labelsep2pt %
\leftmargin\labelwidth %
\advance\leftmargin\labelsep %
\ifdim\baselinestretch pt>1 pt %
\parsep  4pt\relax %
\else   %
\parsep  0pt\relax %
\fi
\itemsep\parsep %
\usecounter{enumiv}%
\let\p@enumiv\@empty
\def\theenumiv{\arabic{enumiv}}%
}%
\let\newblock\relax %
\sloppy\clubpenalty4000\widowpenalty4000
\sfcode`\.=1000\relax
\ifpreprintsty\else\small\fi
}

% Headings, different for even/odd and first.
% Enter TITLE and AUTHORS by hand (!! shift first head if first page even !!)

  \def\AUTHORS{\rmtop CHRISTOPHE CHATELAIN AND BERTRAND BERCHE}
  \def\JOURNAL{PHYSICAL REVIEW E}
  \def\DATE{TO APPEAR DECEMBER 1998}
  \def\TITLE{\rmtop TESTS OF CONFORMAL INVARIANCE IN\dots}
  \def\VOLUME{58}
  \def\NUMBER{6}
  \def\PAGE{1}

\newfont{\rmtop}{cmr10 at 9pt}

  \def\ps@plain{%
  \gdef\@oddhead{\ifnum\thepage=\PAGE {\hbox to 2in{\rmtop\JOURNAL%
  \hfil}\hfil{{\rmtop VOLUME \VOLUME, NUMBER \NUMBER}}\hfil\hbox to %
  2in{\hfil{\rmtop\DATE}}}\else{\hbox to %
  1in{$\underline{\hbox{\rmtop\VOLUME}}$\hfil}\hfil\TITLE\hfil\hbox to %
  1in{\hfil\rmtop\thepage}}\fi}%
  \gdef\@evenhead{\ifnum\thepage=\PAGE {\hbox to 2in{\rmtop\JOURNAL%
  \hfil}\hfil{{\rmtop VOLUME \VOLUME, NUMBER \NUMBER}}\hfil\hbox to %
  2in{\hfil{\rmtop\DATE}}}\else{\hbox to %
  1in{\rmtop\thepage\hfil}\hfil\AUTHORS%
  \hfil\hbox to 1in{\hfil$\underline{\hbox{\rmtop\VOLUME}}$}}\fi}%
  \gdef\@oddfoot{\ifnum\thepage=\PAGE{\hbox to %
  2.5in{\hfil}\hfil$\ \ \underline{\hbox{\rmtop\VOLUME}}\ \ \ \ \ \ %
  ${\rmtop\thepage}%
  \hfil\hbox to 2.5in{\hfil Typeset using REV\TeX}}\else{}\fi}%
  \gdef\@evenfoot{\ifnum\thepage=\PAGE{\hbox to %
  2.5in{\hfil}\hfil$\ \ \underline{\hbox{\rmtop\VOLUME}}\ \ \ \ \ \ %
  ${\rmtop\thepage}%
  \hfil\hbox to 2.5in{\hfil Typeset using REV\TeX}}\else{}\fi}%
  }%


  \makeatother

